How rare are counter Evershed flows?

One of the main characteristics of the penumbra of sunspots is the radially outward-directed Evershed flow. Only recently have penumbral regions been reported with similar characteristics to normal penumbral filaments, but with an opposite direction of the flow. Such flows directed towards the umbra are known as counter Evershed flows (CEFs). We aim to determine the frequency of occurrence of CEFs in active regions (ARs) and to characterize their lifetime and the prevailing conditions in the ARs. We analysed the continuum images, Dopplergrams, and magnetograms recorded by SDO/HMI of 97 ARs that appeared from 2011 to 2017. We followed the ARs for $9.6\pm1.4$ days on average. We found 384 CEFs in total, with a median value of 6 CEFs per AR. CEFs are a rather common feature, they occur in 83.5% of all ARs regardless of the magnetic complexity of the AR. However, CEFs were observed on average only during 5.9% of the mean total duration of all the observations analyzed here. The lifetime of CEFs follows a log-normal distribution with a median value of 10.6$_{-6.0}^{+12.4}$ hr. In addition, we report two populations of CEFs depending on whether they are associated with light bridges, or not. We explain that the rarity of reports of CEFs in the literature is a result of highly incomplete coverage of ARs with spectropolarimetric data. By using the continuous observations now routinely available from space, we are able to overcome this limitation.

==> How rare are Counter Evershed Flows/all_other_CEFs.tex <==

\begin{figure*}[htbp]
 \centering
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR12671a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12671b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12671c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12671d.png}
 \caption{AR\,12671 followed for    8.6 days from 16-Aug-2017 starting at 06:12\,UT.\label{fig:DS00}}
 \end{figure*}


\begin{figure*}[htbp]
 \centering
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR12665a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12665b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12665c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12665d.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12665e.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12665f.png}
 \caption{AR\,12665 followed for    9.4 days from  7-Jul-2017 starting at 12:00\,UT.\label{fig:DS02}}
 \end{figure*}


\begin{figure*}[htbp]
 \centering
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR12599a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12599b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12599c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12599d.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12599e.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12599f.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12599g.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12599h.png}
 \caption{AR\,12599 followed for    9.2 days from  5-Oct-2016 starting at 00:00\,UT.\label{fig:DS05}}
 \end{figure*}


\begin{figure*}[htbp]
 \centering
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR12585a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12585b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12585c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12585d.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12585e.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12585f.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12585g.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12585h.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12585i.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12585j.png}
 \caption{AR\,12585 followed for    9.4 days from  1-Sep-2016 starting at 00:36\,UT.\label{fig:DS06}}
 \end{figure*}


\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}

 \includegraphics[width=.48\textwidth]{CEF_AR12576a.png}
 \caption{AR\,12576 followed for    6.4 days from 10-Aug-2016 starting at 14:36\,UT.\label{fig:DS07}}
 \end{figure*}


\begin{figure*}[htbp]
 \centering
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR12565a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12565b.png}
 \caption{AR\,12565 followed for    8.7 days from 14-Jul-2016 starting at 17:00\,UT.\label{fig:DS09}}
 \end{figure*}


\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR12567a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12567b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12567c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12567d.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12567e.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12567f.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12567g.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12567h.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12567i.png}
 \caption{AR\,12567 followed for   10.6 days from 12-Jul-2016 starting at 19:00\,UT.\label{fig:DS10}}
 \end{figure*}


\begin{figure*}[htbp]
 \centering
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR12542a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12542b.png}
 \caption{AR\,12542 followed for    8.1 days from  5-May-2016 starting at 21:00\,UT.\label{fig:DS13}}
 \end{figure*}


\begin{figure*}[htbp]
 \centering
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR12529a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12529b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12529c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12529d.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12529e.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12529f.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12529g.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12529h.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12529i.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12529j.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12529k.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12529l.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12529m.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12529n.png}
 \caption{AR\,12529 followed for    9.2 days from  9-Apr-2016 starting at 08:00\,UT.\label{fig:DS14}}
 \end{figure*}


\begin{figure*}[htbp]
 \centering
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR12489a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12489b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12489c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12489d.png}
 \caption{AR\,12489 followed for    8.9 days from 26-Jan-2016 starting at 00:00\,UT.\label{fig:DS16}}
 \end{figure*}


\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}

 \includegraphics[width=.48\textwidth]{CEF_AR12483a.png}
 \caption{AR\,12483 followed for    8.6 days from  8-Jan-2016 starting at 10:36\,UT.\label{fig:DS17}}
 \end{figure*}


\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}

 \includegraphics[width=.48\textwidth]{CEF_AR12480a.png}
 \caption{AR\,12480 followed for    9.4 days from  7-Jan-2016 starting at 13:36\,UT.\label{fig:DS18}}
 \end{figure*}


\begin{figure*}[htbp]
 \centering
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR12470a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12470b.png}
 \caption{AR\,12470 followed for   10.9 days from 13-Dec-2015 starting at 21:36\,UT.\label{fig:DS19}}
 \end{figure*}


\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR12381a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12381b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12381c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12381d.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12381e.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12381f.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12381g.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12381h.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12381i.png}
 \caption{AR\,12381 followed for   10.7 days from  5-Jul-2015 starting at 06:12\,UT.\label{fig:DS23}}
 \end{figure*}


\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR12371a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12371b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12371c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12371d.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12371e.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12371f.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12371g.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12371h.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12371i.png}
 \caption{AR\,12371 followed for    9.6 days from 17-Jun-2015 starting at 05:00\,UT.\label{fig:DS24}}
 \end{figure*}


\begin{figure*}[htbp]
 \centering
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR12339a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12339b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12339c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12339d.png}
 \caption{AR\,12339 followed for   10.3 days from  6-May-2015 starting at 08:12\,UT.\label{fig:DS26}}
 \end{figure*}


\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR12321a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12321b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12321c.png}
 \caption{AR\,12321 followed for    9.1 days from 13-Apr-2015 starting at 05:12\,UT.\label{fig:DS27}}
 \end{figure*}


\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR12324a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12324b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12324c.png}
 \caption{AR\,12324 followed for    9.0 days from 14-Apr-2015 starting at 23:12\,UT.\label{fig:DS28}}
 \end{figure*}


\begin{figure*}[htbp]
 \centering
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR12325a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12325b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12325c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12325d.png}
 \caption{AR\,12325 followed for    9.4 days from 15-Apr-2015 starting at 06:24\,UT.\label{fig:DS29}}
 \end{figure*}


\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR12305a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12305b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12305c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12305d.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12305e.png}
 \caption{AR\,12305 followed for    9.9 days from 22-Mar-2015 starting at 07:00\,UT.\label{fig:DS30}}
 \end{figure*}


\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR12282a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12282b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12282c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12282d.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12282e.png}
 \caption{AR\,12282 followed for   10.5 days from  8-Feb-2015 starting at 23:24\,UT.\label{fig:DS32}}
 \end{figure*}


\begin{figure*}[htbp]
 \centering
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR12277a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12277b.png}
 \caption{AR\,12277 followed for   10.2 days from 30-Jan-2015 starting at 02:48\,UT.\label{fig:DS33}}
 \end{figure*}


\begin{figure*}[htbp]
 \centering
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR12268a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12268b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12268c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12268d.png}
 \caption{AR\,12268 followed for   10.6 days from 22-Jan-2015 starting at 21:48\,UT.\label{fig:DS34}}
 \end{figure*}


\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}

 \includegraphics[width=.48\textwidth]{CEF_AR12259a.png}
 \caption{AR\,12259 followed for   11.6 days from  8-Jan-2015 starting at 13:24\,UT.\label{fig:DS36}}
 \end{figure*}


\begin{figure*}[htbp]
 \centering
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR12257a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12257b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12257c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12257d.png}
 \caption{AR\,12257 followed for    6.8 days from  6-Jan-2015 starting at 13:36\,UT.\label{fig:DS37}}
 \end{figure*}


\clearpage
\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR12241a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12241b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12241c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12241d.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12241e.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12241f.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12241g.png}
 \caption{AR\,12241 followed for    8.8 days from 15-Dec-2014 starting at 03:12\,UT.\label{fig:DS38}}
 \end{figure*}


\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR12237a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12237b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12237c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12237d.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12237e.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12237f.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12237g.png}
 \caption{AR\,12237 followed for    8.2 days from 13-Dec-2014 starting at 23:00\,UT.\label{fig:DS39}}
 \end{figure*}


\begin{figure*}[htbp]
 \centering
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR12236a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12236b.png}
 \caption{AR\,12236 followed for   10.0 days from 12-Dec-2014 starting at 02:00\,UT.\label{fig:DS40}}
 \end{figure*}


\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}

 \includegraphics[width=.48\textwidth]{CEF_AR12230a.png}
 \caption{AR\,12230 followed for    7.4 days from  8-Dec-2014 starting at 15:00\,UT.\label{fig:DS41}}
 \end{figure*}


\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR12222a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12222b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12222c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12222d.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12222e.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12222f.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12222g.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12222h.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12222i.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12222j.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12222k.png}
 \caption{AR\,12222 followed for    8.8 days from 27-Nov-2014 starting at 20:00\,UT.\label{fig:DS43}}
 \end{figure*}


\begin{figure*}[htbp]
 \centering
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR12216a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12216b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12216c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12216d.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12216e.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12216f.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12216g.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12216h.png}
 \caption{AR\,12216 followed for    9.6 days from 21-Nov-2014 starting at 00:24\,UT.\label{fig:DS45}}
 \end{figure*}


\begin{figure*}[htbp]
 \centering
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR12209a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12209b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12209c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12209d.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12209e.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12209f.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12209g.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12209h.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12209i.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12209j.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12209k.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12209l.png}
 \caption{AR\,12209 followed for    9.9 days from 15-Nov-2014 starting at 18:12\,UT.\label{fig:DS46}}
 \end{figure*}


\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}

 \includegraphics[width=.48\textwidth]{CEF_AR12187a.png}
 \caption{AR\,12187 followed for   10.2 days from 12-Oct-2014 starting at 21:00\,UT.\label{fig:DS48}}
 \end{figure*}


\begin{figure*}[htbp]
 \centering
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR12178a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12178b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12178c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12178d.png}
 \caption{AR\,12178 followed for   10.4 days from 28-Sep-2014 starting at 02:36\,UT.\label{fig:DS50}}
 \end{figure*}


\begin{figure*}[htbp]
 \centering
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR12175a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12175b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12175c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12175d.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12175e.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12175f.png}
 \caption{AR\,12175 followed for    6.2 days from 24-Sep-2014 starting at 19:48\,UT.\label{fig:DS51}}
 \end{figure*}


\begin{figure*}[htbp]
 \centering
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR12172a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12172b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12172c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12172d.png}
 \caption{AR\,12172 followed for    8.3 days from 22-Sep-2014 starting at 12:00\,UT.\label{fig:DS52}}
 \end{figure*}


\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR12158a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12158b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12158c.png}
 \caption{AR\,12158 followed for   10.6 days from  5-Sep-2014 starting at 18:36\,UT.\label{fig:DS53}}
 \end{figure*}


\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}

 \includegraphics[width=.48\textwidth]{CEF_AR12149a.png}
 \caption{AR\,12149 followed for   10.5 days from 22-Aug-2014 starting at 07:12\,UT.\label{fig:DS55}}
 \end{figure*}


\begin{figure*}[htbp]
 \centering
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR12146a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12146b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12146c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12146d.png}
 \caption{AR\,12146 followed for   10.6 days from 17-Aug-2014 starting at 12:00\,UT.\label{fig:DS56}}
 \end{figure*}


\begin{figure*}[htbp]
 \centering
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR12135a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12135b.png}
 \caption{AR\,12135 followed for   10.4 days from  6-Aug-2014 starting at 10:48\,UT.\label{fig:DS57}}
 \end{figure*}


\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR12109a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12109b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12109c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12109d.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12109e.png}
 \caption{AR\,12109 followed for   11.1 days from  3-Jul-2014 starting at 03:24\,UT.\label{fig:DS58}}
 \end{figure*}


\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR12108a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12108b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12108c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12108d.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12108e.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12108f.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12108g.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12108h.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12108i.png}
 \caption{AR\,12108 followed for    9.9 days from  2-Jul-2014 starting at 06:24\,UT.\label{fig:DS59}}
 \end{figure*}


\begin{figure*}[htbp]
 \centering
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR12085a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12085b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12085c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12085d.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12085e.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12085f.png}
 \caption{AR\,12085 followed for    7.1 days from  6-Jun-2014 starting at 11:24\,UT.\label{fig:DS62}}
 \end{figure*}


\begin{figure*}[htbp]
 \centering
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR12082a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12082b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12082c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12082d.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12082e.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12082f.png}
 \caption{AR\,12082 followed for    8.2 days from  5-Jun-2014 starting at 08:24\,UT.\label{fig:DS63}}
 \end{figure*}


\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR12080a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12080b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12080c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12080d.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12080e.png}
 \caption{AR\,12080 followed for    8.8 days from  4-Jun-2014 starting at 19:24\,UT.\label{fig:DS64}}
 \end{figure*}


\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}

 \includegraphics[width=.48\textwidth]{CEF_AR12056a.png}
 \caption{AR\,12056 followed for   10.5 days from  6-May-2014 starting at 21:48\,UT.\label{fig:DS65}}
 \end{figure*}


\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR12055a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12055b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12055c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12055d.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12055e.png}
 \caption{AR\,12055 followed for   10.2 days from  6-May-2014 starting at 01:48\,UT.\label{fig:DS66}}
 \end{figure*}


\begin{figure*}[htbp]
 \centering
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR12049a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12049b.png}
 \caption{AR\,12049 followed for   10.9 days from 27-Apr-2014 starting at 22:12\,UT.\label{fig:DS67}}
 \end{figure*}


\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR12034a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12034b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR12034c.png}
 \caption{AR\,12034 followed for    9.6 days from 11-Apr-2014 starting at 09:00\,UT.\label{fig:DS68}}
 \end{figure*}


\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}

 \includegraphics[width=.48\textwidth]{CEF_AR12005a.png}
 \caption{AR\,12005 followed for   10.5 days from 13-Mar-2014 starting at 02:00\,UT.\label{fig:DS70}}
 \end{figure*}


\begin{figure*}[htbp]
 \centering
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR11976a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11976b.png}
 \caption{AR\,11976 followed for   11.4 days from  9-Feb-2014 starting at 03:12\,UT.\label{fig:DS72}}
 \end{figure*}


\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR11960a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11960b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11960c.png}
 \caption{AR\,11960 followed for   11.4 days from 19-Jan-2014 starting at 03:00\,UT.\label{fig:DS74}}
 \end{figure*}


\begin{figure*}[htbp]
 \centering
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR11944a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11944b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11944c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11944d.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11944e.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11944f.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11944g.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11944h.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11944i.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11944j.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11944k.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11944l.png}
 \caption{AR\,11944 followed for    8.3 days from  3-Jan-2014 starting at 22:12\,UT.\label{fig:DS75}}
 \end{figure*}


\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR11899a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11899b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11899c.png}
 \caption{AR\,11899 followed for   10.8 days from 13-Nov-2013 starting at 07:48\,UT.\label{fig:DS78}}
 \end{figure*}


\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR11893a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11893b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11893c.png}
 \caption{AR\,11893 followed for   10.5 days from  8-Nov-2013 starting at 12:36\,UT.\label{fig:DS79}}
 \end{figure*}


\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR11890a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11890b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11890c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11890d.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11890e.png}
 \caption{AR\,11890 followed for    6.5 days from  4-Nov-2013 starting at 12:00\,UT.\label{fig:DS80}}
 \end{figure*}


\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR11877a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11877b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11877c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11877d.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11877e.png}
 \caption{AR\,11877 followed for   10.5 days from 19-Oct-2013 starting at 15:00\,UT.\label{fig:DS81}}
 \end{figure*}


\begin{figure*}[htbp]
 \centering
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR11875a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11875b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11875c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11875d.png}
 \caption{AR\,11875 followed for   10.7 days from 18-Oct-2013 starting at 00:00\,UT.\label{fig:DS82}}
 \end{figure*}


\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR11861a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11861b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11861c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11861d.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11861e.png}
 \caption{AR\,11861 followed for    8.1 days from  9-Oct-2013 starting at 22:48\,UT.\label{fig:DS83}}
 \end{figure*}


\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR11818a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11818b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11818c.png}
 \caption{AR\,11818 followed for    9.2 days from 11-Aug-2013 starting at 10:00\,UT.\label{fig:DS84}}
 \end{figure*}


\begin{figure*}[htbp]
 \centering
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR11734a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11734b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11734c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11734d.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11734e.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11734f.png}
 \caption{AR\,11734 followed for   10.0 days from  1-May-2013 starting at 01:00\,UT.\label{fig:DS85}}
 \end{figure*}


\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR11711a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11711b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11711c.png}
 \caption{AR\,11711 followed for   10.7 days from 31-Mar-2013 starting at 01:48\,UT.\label{fig:DS87}}
 \end{figure*}


\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR11654a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11654b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11654c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11654d.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11654e.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11654f.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11654g.png}
 \caption{AR\,11654 followed for   10.0 days from  8-Jan-2013 starting at 15:00\,UT.\label{fig:DS90}}
 \end{figure*}


\begin{figure*}[htbp]
 \centering
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR11640a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11640b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11640c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11640d.png}
 \caption{AR\,11640 followed for    7.7 days from 30-Dec-2012 starting at 02:00\,UT.\label{fig:DS91}}
 \end{figure*}


\begin{figure*}[htbp]
 \centering
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR11623a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11623b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11623c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11623d.png}
 \caption{AR\,11623 followed for   11.1 days from 28-Nov-2012 starting at 00:12\,UT.\label{fig:DS92}}
 \end{figure*}


\clearpage

\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR11598a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11598b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11598c.png}
 \caption{AR\,11598 followed for   11.1 days from 22-Oct-2012 starting at 00:00\,UT.\label{fig:DS93}}
 \end{figure*}

\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}

 \includegraphics[width=.48\textwidth]{CEF_AR11596a.png}
 \caption{AR\,11596 followed for   11.1 days from 18-Oct-2012 starting at 18:48\,UT.\label{fig:DS94}}
 \end{figure*}


\begin{figure*}[htbp]
 \centering
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR11543a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11543b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11543c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11543d.png}
 \caption{AR\,11543 followed for   11.0 days from  8-Aug-2012 starting at 00:24\,UT.\label{fig:DS96}}
 \end{figure*}


\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR11520a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11520b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11520c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11520d.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11520e.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11520f.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11520g.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11520h.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11520i.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11520j.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11520k.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11520l.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11520m.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11520n.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11520o.png}
 \caption{AR\,11520 followed for    8.0 days from  8-Jul-2012 starting at 18:12\,UT.\label{fig:DS97}}
 \end{figure*}


\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR11515a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11515b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11515c.png}
 \caption{AR\,11515 followed for   10.5 days from 27-Jun-2012 starting at 20:36\,UT.\label{fig:DS98}}
 \end{figure*}


\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}

 \includegraphics[width=.48\textwidth]{CEF_AR11513a.png}
 \caption{AR\,11513 followed for   11.3 days from 26-Jun-2012 starting at 17:12\,UT.\label{fig:DS99}}
 \end{figure*}


\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR11504a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11504b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11504c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11504d.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11504e.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11504f.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11504g.png}
 \caption{AR\,11504 followed for   11.3 days from  9-Jun-2012 starting at 10:24\,UT.\label{fig:DS100}}
 \end{figure*}


\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR11476a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11476b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11476c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11476d.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11476e.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11476f.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11476g.png}
 \caption{AR\,11476 followed for    8.0 days from  8-May-2012 starting at 00:00\,UT.\label{fig:DS101}}
 \end{figure*}


\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR11460a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11460b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11460c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11460d.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11460e.png}
 \caption{AR\,11460 followed for    8.5 days from 16-Apr-2012 starting at 19:24\,UT.\label{fig:DS103}}
 \end{figure*}


\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR11384a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11384b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11384c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11384d.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11384e.png}
 \caption{AR\,11384 followed for   11.4 days from 20-Dec-2011 starting at 03:36\,UT.\label{fig:DS105}}
 \end{figure*}


\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR11339a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11339b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11339c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11339d.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11339e.png}
 \caption{AR\,11339 followed for   11.6 days from  2-Nov-2011 starting at 10:00\,UT.\label{fig:DS106}}
 \end{figure*}


\begin{figure*}[htbp]
 \centering
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR11330a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11330b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11330c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11330d.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11330e.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11330f.png}
 \caption{AR\,11330 followed for   10.1 days from 22-Oct-2011 starting at 16:36\,UT.\label{fig:DS107}}
 \end{figure*}


\begin{figure*}[htbp]
 \centering
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR11314a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11314b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11314c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11314d.png}
 \caption{AR\,11314 followed for    8.7 days from 11-Oct-2011 starting at 11:36\,UT.\label{fig:DS108}}
 \end{figure*}


\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR11302a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11302b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11302c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11302d.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11302e.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11302f.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11302g.png}
 \caption{AR\,11302 followed for   11.1 days from 23-Sep-2011 starting at 05:24\,UT.\label{fig:DS110}}
 \end{figure*}


\begin{figure*}[htbp]
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR11289a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11289b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11289c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11289d.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11289e.png}
 \caption{AR\,11289 followed for   10.3 days from  8-Sep-2011 starting at 06:12\,UT.\label{fig:DS111}}
 \end{figure*}


\begin{figure*}[htbp]
 \centering
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{colorbars.pdf}
 \includegraphics[width=.48\textwidth]{CEF_AR11263a.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11263b.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11263c.png}
 \includegraphics[width=.48\textwidth]{CEF_AR11263d.png}
 \caption{AR\,11263 followed for    9.5 days from 30-Jul-2011 starting at 00:12\,UT.\label{fig:DS112}}
 \end{figure*}



==> How rare are Counter Evershed Flows/table_all_cefs_letter.tex <==
\longtab{
{\scriptsize
\begin{landscape}
\begin{longtable}{rcccccccclcrrrrrrrrrrrrl}
\caption{Parameters of the observations and of the observed ARs that hosted CEFs.\\ {\tiny \textbf{Notes.} \tablefoottext{a}{NOAA AR number.} \tablefoottext{b}{Starting observation day.} \tablefoottext{c}{Starting time.}  \tablefoottext{d}{Total duration of the observation.} \tablefoottext{e}{Size of the FoV in arcsec.} \tablefoottext{f}{Median latitude of the AR.} \tablefoottext{g,h}{Longitude of the AR when the observations started\tablefoottext{g} and ended.\tablefoottext{h}} \tablefoottext{i}{Median corrected area of the AR in millionths of the solar hemisphere.} \tablefoottext{j}{Number of detected CEFs per AR.}  \tablefoottext{k}{Magnetic classification of the AR of the day. Roman numbers denote the day of the observation starting from the first day, indicated by (I) to (XII). For the days with CEFs, the  magnetic classification is preceded by three numbers: The first number counts how many CEFs appear on that day. The second number inside circular parentheses displays how many CEFs reached their maximum area on that particular day. The last number inside squared parentheses marks how many CEFs disappeared on that day. \tablefoottext{l}{Figure about the AR.}} }  }\label{tab:OtherCEFs}\\
\midrule[1.5pt]
\multirow{2}{*}{ID}&NOAA& \multirow{2}{*}{Date}\tablefootmark{(b)} & \multirow{2}{*}{Time}\tablefootmark{(c)}& $\Delta t_{\rm Obs}$\tablefootmark{(d)} & FoV\tablefootmark{(e)} & {$\phi$}\tablefootmark{(f)} & {$\lambda_{\rm start}$}\tablefootmark{(g)}& {$\lambda_{\rm end}$}\tablefootmark{(h)} & Area\tablefootmark{(i)} & Total &\multicolumn{12}{c}{Magnetic classification of the day \tablefootmark{(k)}} & \multirow{2}{*}{Fig.}\tablefootmark{(l)} \\
&AR\tablefootmark{(a)} & & &(hr)& (\arcsec{})& (deg) & (deg) & (deg) & (MSH)& CEFs\tablefootmark{(j)} & (I)& (II)&(III) &(IV) &(V) &(VI) &(VII) &(VIII) &(IX) &(X) &(XI) &(XII) &\\
\bottomrule[1.5pt]
\endfirsthead
\caption{continued.}\\
\toprule[1.5pt]
\multirow{2}{*}{ID}&NOAA& \multirow{2}{*}{Date}\tablefootmark{(b)} & \multirow{2}{*}{Time}\tablefootmark{(c)}& $\Delta t_{\rm Obs}$\tablefootmark{(d)} & FoV\tablefootmark{(e)} & {$\phi$}\tablefootmark{(f)} & {$\lambda_{\rm start}$}\tablefootmark{(g)}& {$\lambda_{\rm end}$}\tablefootmark{(h)} & Area\tablefootmark{(i)} & Total &\multicolumn{12}{c}{Magnetic classification of the day \tablefootmark{(k)}} & \multirow{2}{*}{Fig.}\tablefootmark{(l)} \\
&AR\tablefootmark{(a)} & & &(hr)& (\arcsec{})& (deg) & (deg) & (deg) & (MSH)& CEFs\tablefootmark{(j)} & (I)& (II)&(III) &(IV) &(V) &(VI) &(VII) &(VIII) &(IX) &(X) &(XI) &(XII) &\\
\midrule[1.5pt]
\endhead
\bottomrule[1.5pt]
\endfoot
  1& 12670& 2017-08-07& 16:30& 217.8& 120$\times$120& S06& E59& W61& 140$^{+30}_{-10}$&  0& $\beta$& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\cdots$& $\cdots$& \ref{fig:arswithoutcefs}a\\
  2& 12664& 2017-06-26& 18:30& 221.8& 120$\times$120& N18& E60& W60&  70$^{+20}_{-20}$&  0& $\alpha$& $\alpha$& $\alpha$& $\beta$& $\beta$& $\beta\gamma$& $\beta$& $\beta$& $\beta$& $\alpha$& $\cdots$& $\cdots$& \ref{fig:arswithoutcefs}b\\
  3& 12600& 2016-10-12& 11:30& 217.8& 120$\times$130& N11& E60& W59&  90$^{+30}_{-10}$&  0& $\alpha$& $\alpha$& $\beta$& $\beta$& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\cdots$& $\cdots$& \ref{fig:arswithoutcefs}c\\
  4& 12574& 2016-08-13& 20:00& 177.2& 110$\times$140& N05& E42& W55& 200$^{+80}_{-40}$&  0& $\beta$& $\beta$& $\beta$& $\beta$& $\beta$& $\beta$& $\beta$& $\alpha$& $\cdots$& $\cdots$& $\cdots$& $\cdots$& \ref{fig:arswithoutcefs}d\\
  5& 12526& 2016-03-30& 10:18& 283.8& 170$\times$140& S05& E72& W84& 190$^{+40}_{-10}$&  0& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\beta$& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\alpha$& \ref{fig:arswithoutcefs}e\\
  6& 12341& 2015-05-13& 18:41& 252.8& 150$\times$135& S19& E68& W68&  70$^{+10}_{-20}$&  0& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\cdots$& \ref{fig:arswithoutcefs}f\\
  7& 12227& 2014-12-08& 15:43& 237.6& 140$\times$130& S04& E69& W62& 120$^{+40}_{-30}$&  0& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\beta$& $\beta$& $\beta$& $\beta$& $\alpha$& $\cdots$& \ref{fig:arswithoutcefs}g\\
  8& 12218& 2014-11-30& 08:40& 218.4& 130$\times$120& N16& E58& W61& 140$^{+10}_{-20}$&  0& $\beta$& $\beta$& $\beta$& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\cdots$& $\cdots$& \ref{fig:arswithoutcefs}h\\
  9& 12186& 2014-10-13& 16:29& 228.6& 130$\times$120& S20& E60& W63& 170$^{+20}_{-30}$&  0& $\alpha$& $\beta$& $\beta$& $\beta$& $\beta$& $\beta$& $\beta$& $\beta$& $\alpha$& $\beta$& $\alpha$& $\cdots$& \ref{fig:arswithoutcefs}i\\
 10& 12151& 2014-08-29& 09:53& 259.2& 170$\times$130& S07& E73& W70& 110$^{+20}_{-30}$&  0& $\alpha$& $\alpha$& $\beta$& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\beta$& $\alpha$& $\alpha$& $\cdots$& \ref{fig:arswithoutcefs}j\\
 11& 12107& 2014-07-05& 23:10& 268.8& 230$\times$150& S20& E69& W76& 250$^{+50}_{-60}$&  0& $\beta$& $\beta\gamma$& $\beta\delta$& $\beta$& $\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\beta$& $\beta$& $\alpha$& $\alpha$& \ref{fig:arswithoutcefs}k\\
 12& 12032& 2014-04-13& 21:21& 238.8& 140$\times$150& N13& E63& W68& 150$^{+40}_{-10}$&  0& $\beta$& $\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\alpha$& $\alpha$& $\beta$& $\alpha$& $\alpha$& $\cdots$& $\cdots$& \ref{fig:arswithoutcefs}l\\
 13& 11931& 2013-12-24& 17:55&  86.2& 125$\times$120& S15& E65& W72& 190$^{+50}_{-30}$&  0& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\beta$& $\beta$& $\alpha$& $\cdots$& \ref{fig:arswithoutcefs}m\\
 14& 11692& 2013-03-15& 19:18& 244.6& 180$\times$195& N09& E62& W72& 220$^{+30}_{-20}$&  0& $\alpha$& $\alpha$& $\alpha$& $\beta$& $\alpha$& $\alpha$& $\alpha$& $\beta$& $\beta$& $\beta$& $\beta$& $\cdots$& \ref{fig:arswithoutcefs}n\\
 15& 11582& 2012-10-02& 07:32& 265.8& 170$\times$170& S12& E73& W73& 270$^{+50}_{-80}$&  0& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\beta$& $\beta$& $\alpha$& $\alpha$& $\alpha$& $\cdots$& \ref{fig:arswithoutcefs}o\\
 16& 11312& 2011-10-11& 00:00& 285.8& 160$\times$125& N23& E76& W78& 210$^{+20}_{-60}$&  0& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\beta$& $\alpha$& $\alpha$& $\alpha$& \ref{fig:arswithoutcefs}p\\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\toprule[1.5pt]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 17& 12671& 2017-08-16& 21:24& 205.6& 400$\times$150& N11& E59& W54&  360$^{+140}_{- 50}$&  4& \textbf{2}(\textbf{1})[\textbf{1}]$\beta$& (\textbf{1})[\textbf{1}]$\beta\gamma\delta$& $\beta\gamma$& \textbf{2}(\textbf{2})[\textbf{2}]$\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\cdots$& $\cdots$& $\cdots$& \ref{fig:DS00}\\
 18& 12665& 2017-07-09& 21:36& 226.8& 390$\times$270& S06& E57& W68&  480$^{+170}_{-210}$&  6& $\beta$& $\beta$& \textbf{1}(\textbf{1})$\beta$& [\textbf{1}]$\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\beta$& \textbf{4}(\textbf{2})[\textbf{2}]$\beta$& (\textbf{2})$\beta$& \textbf{1}(\textbf{1})[\textbf{3}]$\beta$& $\cdots$& $\cdots$& \ref{fig:DS02}\\
 19& 12599& 2016-10-05& 05:36& 221.8& 125$\times$110& S15& E58& W64&  400$^{+210}_{- 10}$&  8& \textbf{1}(\textbf{1})[\textbf{1}]$\beta$& \textbf{1}$\beta$& (\textbf{1})[\textbf{1}]$\alpha$& $\alpha$& $\beta$& \textbf{1}$\beta$& \textbf{2}(\textbf{3})[\textbf{2}]$\beta$& \textbf{3}(\textbf{3})[\textbf{3}]$\beta$& [\textbf{1}]$\beta$& $\beta$& $\cdots$& $\cdots$& \ref{fig:DS05}\\
 20& 12585& 2016-09-01& 08:48& 225.8& 240$\times$120& N08& E70& W55&  430$^{+ 50}_{-120}$& 10& \textbf{3}(\textbf{2})[\textbf{1}]$\beta$& \textbf{2}(\textbf{2})[\textbf{3}]$\beta$& \textbf{2}(\textbf{2})[\textbf{2}]$\beta\gamma$& \textbf{1}(\textbf{2})[\textbf{2}]$\beta\gamma$& $\beta\gamma$& $\beta$& $\beta\gamma$& \textbf{1}$\beta\gamma$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta\delta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta\delta$& $\cdots$& $\cdots$& \ref{fig:DS06}\\
 21& 12576& 2016-08-15& 08:00& 153.2&  60$\times$ 50& S12& E55& W29&  130$^{+ 30}_{- 10}$&  1& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\alpha$& \textbf{1}(\textbf{1})[\textbf{1}]$\alpha$& $\alpha$& $\cdots$& $\cdots$& $\cdots$& $\cdots$& $\cdots$& \ref{fig:DS07}\\
 22& 12565& 2016-07-21& 04:00& 207.8& 145$\times$120& N04& E36& W78&  300$^{+ 80}_{- 20}$&  2& $\alpha$& $\beta$& $\beta$& $\beta$& $\beta$& \textbf{1}$\beta$& $\beta$& \textbf{1}(\textbf{2})[\textbf{2}]$\beta$& $\alpha$& $\alpha$& $\cdots$& $\cdots$& \ref{fig:DS09}\\
 23& 12567& 2016-07-15& 21:00& 253.8& 230$\times$135& N05& E71& W69&  330$^{+140}_{- 60}$&  9& $\beta$& \textbf{2}(\textbf{2})$\beta\gamma$& \textbf{1}(\textbf{1})[\textbf{3}]$\beta\gamma\delta$& $\beta\gamma$& $\beta\gamma$& \textbf{3}(\textbf{3})[\textbf{1}]$\beta\gamma$& \textbf{3}(\textbf{2})[\textbf{4}]$\beta$& (\textbf{1})$\beta\gamma$& [\textbf{1}]$\beta$& $\cdots$& $\cdots$& $\cdots$& \ref{fig:DS10}\\
 24& 12542& 2016-05-06& 17:12& 194.8& 135$\times$140& N11& E57& W49&  150$^{+ 30}_{- 20}$&  2& $\beta$& \textbf{1}(\textbf{1})$\beta$& [\textbf{1}]$\beta$& $\alpha$& $\beta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta\gamma$& $\beta\gamma$& $\beta$& $\beta\gamma$& $\beta$& $\cdots$& $\cdots$& \ref{fig:DS13}\\
 25& 12529& 2016-04-09& 11:48& 219.8& 170$\times$140& N10& E60& W60&  790$^{+ 70}_{- 30}$& 14& \textbf{1}(\textbf{1})[\textbf{1}]$\beta$& \textbf{3}(\textbf{3})[\textbf{1}]$\beta$& \textbf{2}(\textbf{2})[\textbf{4}]$\beta$& \textbf{3}(\textbf{3})[\textbf{2}]$\beta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta$& [\textbf{1}]$\beta$& \textbf{1}(\textbf{1})$\beta$& \textbf{2}[\textbf{1}]$\beta\gamma$& \textbf{1}(\textbf{3})[\textbf{3}]$\beta\gamma$& $\beta\gamma$& $\cdots$& $\cdots$& \ref{fig:DS14}\\
 26& 12489& 2016-01-26& 18:36& 213.8& 310$\times$185& N10& E53& W65&  250$^{+150}_{- 50}$&  4& \textbf{1}(\textbf{1})[\textbf{1}]$\beta$& \textbf{1}(\textbf{1})$\beta$& [\textbf{1}]$\beta$& $\beta$& $\beta$& $\beta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta$& $\alpha$& $\cdots$& $\cdots$& $\cdots$& \ref{fig:DS16}\\
 27& 12483& 2016-01-11& 02:24& 205.2& 240$\times$130& N17& E51& W61&   90$^{+ 80}_{- 50}$&  1& $\beta$& $\beta$& \textbf{1}$\beta$& (\textbf{1})[\textbf{1}]$\beta$& $\beta$& $\beta$& $\beta$& $\beta$& $\alpha$& $\cdots$& $\cdots$& $\cdots$& \ref{fig:DS17}\\
 28& 12480& 2016-01-13& 00:24& 226.2& 295$\times$110& N03& E65& W59&  170$^{+ 40}_{- 10}$&  1& $\beta$& $\beta$& $\beta$& $\beta$& $\beta$& \textbf{1}$\beta$& (\textbf{1})[\textbf{1}]$\beta$& $\beta$& $\alpha$& $\alpha$& $\cdots$& $\cdots$& \ref{fig:DS18}\\
 29& 12470& 2015-12-15& 02:24& 262.2& 390$\times$280& N14& E72& W71&  430$^{+160}_{-180}$&  2& $\alpha$& \textbf{1}$\beta$& (\textbf{1})[\textbf{1}]$\beta$& \textbf{1}$\beta$& (\textbf{1})[\textbf{1}]$\beta$& $\beta$& $\beta$& $\beta$& $\beta$& $\beta$& $\alpha$& $\alpha$& \ref{fig:DS19}\\
 30& 12381& 2015-07-05& 23:48& 257.6& 350$\times$170& N15& E53& W88&  360$^{+260}_{-140}$&  9& \textbf{3}(\textbf{1})$\beta$& \textbf{2}(\textbf{3})[\textbf{2}]$\beta$& \textbf{1}(\textbf{2})[\textbf{3}]$\beta\gamma$& [\textbf{1}]$\beta\gamma$& \textbf{1}$\beta$& (\textbf{1})[\textbf{1}]$\beta$& \textbf{1}(\textbf{1})$\beta$& [\textbf{1}]$\beta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta$& $\beta$& $\beta$& $\cdots$& \ref{fig:DS23}\\
 31& 12371& 2015-06-17& 15:24& 230.8& 360$\times$200& N12& E64& W62&  950$^{+430}_{-170}$&  9& \textbf{1}(\textbf{1})$\beta$& \textbf{2}(\textbf{1})[\textbf{1}]$\beta\gamma$& \textbf{1}(\textbf{1})[\textbf{2}]$\beta\gamma\delta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta\gamma\delta$& (\textbf{1})[\textbf{1}]$\beta\gamma\delta$& $\beta\gamma\delta$& \textbf{1}(\textbf{1})$\beta\gamma\delta$& \textbf{2}(\textbf{2})[\textbf{2}]$\beta\gamma\delta$& \textbf{1}(\textbf{1})[\textbf{2}]$\beta\gamma$& $\beta\gamma$& $\cdots$& $\cdots$& \ref{fig:DS24}\\
 32& 12339& 2015-05-08& 17:00& 246.0& 405$\times$170& N13& E70& W65&  670$^{+360}_{-170}$&  4& $\beta\gamma$& $\beta\gamma$& \textbf{2}(\textbf{1})$\beta\gamma$& (\textbf{1})[\textbf{2}]$\beta\gamma$& $\beta\gamma$& \textbf{1}$\beta\gamma$& \textbf{1}(\textbf{2})[\textbf{1}]$\beta\gamma$& [\textbf{1}]$\beta\gamma$& $\beta\gamma$& $\beta$& $\beta\gamma$& $\cdots$& \ref{fig:DS26}\\
 33& 12321& 2015-04-13& 08:12& 218.8& 310$\times$190& N12& E54& W65&  380$^{+300}_{-240}$&  3& \textbf{1}(\textbf{1})[\textbf{1}]$\beta\gamma\delta$& $\beta\gamma\delta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta\gamma$& $\beta\gamma$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\beta$& $\alpha$& $\cdots$& $\cdots$& \ref{fig:DS27}\\
 34& 12324& 2015-04-16& 09:24& 216.6& 175$\times$130& N19& E61& W56&  300$^{+130}_{- 90}$&  3& $\beta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta$& \textbf{2}(\textbf{2})[\textbf{2}]$\beta\gamma$& $\beta$& $\beta\gamma$& $\beta$& $\beta$& $\beta$& $\beta$& $\cdots$& $\cdots$& $\cdots$& \ref{fig:DS28}\\
 35& 12325& 2015-04-17& 11:36& 224.8& 215$\times$130& N05& E68& W56&  205$^{+ 65}_{- 15}$&  4& $\alpha$& $\beta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta$& $\beta$& $\beta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta$& \textbf{1}(\textbf{1})$\beta$& [\textbf{1}]$\beta$& $\alpha$& $\cdots$& $\cdots$& \ref{fig:DS29}\\
 36& 12305& 2015-03-22& 14:00& 238.4& 320$\times$160& S08& E67& W64&  340$^{+120}_{- 70}$&  5& \textbf{1}(\textbf{1})[\textbf{1}]$\beta$& $\beta\gamma$& $\beta\gamma$& $\beta\gamma\delta$& $\beta\gamma\delta$& $\beta\gamma$& \textbf{2}(\textbf{1})$\beta\gamma$& (\textbf{1})[\textbf{2}]$\beta\gamma$& \textbf{2}(\textbf{1})[\textbf{1}]$\beta$& (\textbf{1})$\beta$& [\textbf{1}]$\beta$& $\cdots$& \ref{fig:DS30}\\
 37& 12282& 2015-02-14& 09:24& 252.8& 265$\times$200& N11& E72& W67&  210$^{+120}_{- 30}$&  5& $\alpha$& $\beta$& $\beta$& $\beta\gamma$& $\beta$& $\beta\gamma$& \textbf{3}(\textbf{3})[\textbf{3}]$\beta\gamma$& $\beta\gamma$& $\beta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta$& $\beta$& \ref{fig:DS32}\\
 38& 12277& 2015-02-01& 04:48& 245.8& 180$\times$140& N08& E71& W63&  400$^{+200}_{- 90}$&  2& $\beta\gamma$& $\beta\gamma$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta\gamma$& $\beta\gamma$& \textbf{1}$\beta$& (\textbf{1})[\textbf{1}]$\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\cdots$& \ref{fig:DS33}\\
 39& 12268& 2015-01-23& 20:36& 254.8& 410$\times$190& S10& E77& W63&  430$^{+110}_{- 70}$&  4& \textbf{1}(\textbf{1})[\textbf{1}]$\beta$& \textbf{1}$\beta\gamma$& (\textbf{1})[\textbf{1}]$\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\beta\gamma$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta\gamma$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\cdots$& \ref{fig:DS34}\\
 40& 12259& 2015-01-12& 08:24& 277.8& 190$\times$150& S16& E75& W76&  260$^{+170}_{- 90}$&  1& $\beta$& $\beta\gamma$& \textbf{1}$\beta\gamma$& (\textbf{1})[\textbf{1}]$\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\beta\gamma\delta$& $\beta\delta$& $\beta\gamma$& $\beta$& $\beta$& $\alpha$& \ref{fig:DS36}\\
 41& 12257& 2015-01-08& 18:24& 163.0& 250$\times$150& N07& E17& W73&  380$^{+340}_{- 90}$&  4& $\beta$& $\beta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta$& \textbf{2}(\textbf{2})[\textbf{2}]$\beta$& \textbf{1}(\textbf{1})$\beta\delta$& [\textbf{1}]$\beta\delta$& $\beta\gamma\delta$& $\beta\gamma\delta$& $\cdots$& $\cdots$& $\cdots$& $\cdots$& \ref{fig:DS37}\\
 42& 12241& 2014-12-15& 05:24& 211.8& 320$\times$210& S10& E57& W59&  450$^{+300}_{-210}$&  7& \textbf{3}(\textbf{3})[\textbf{1}]$\beta\gamma$& \textbf{3}(\textbf{1})[\textbf{2}]$\beta\gamma$& (\textbf{2})[\textbf{3}]$\beta\gamma$& $\beta\gamma\delta$& $\beta\gamma\delta$& $\beta\gamma\delta$& \textbf{1}(\textbf{1})$\beta\gamma\delta$& [\textbf{1}]$\beta\gamma\delta$& $\beta\gamma$& $\cdots$& $\cdots$& $\cdots$& \ref{fig:DS38}\\
 43& 12237& 2014-12-15& 22:00& 196.0& 375$\times$220& S13& E49& W57&   40$^{+ 20}_{- 50}$&  7& $\beta$& $\beta$& \textbf{2}(\textbf{2})$\beta$& \textbf{2}(\textbf{2})[\textbf{3}]$\alpha$& [\textbf{1}]$\alpha$& \textbf{2}(\textbf{2})[\textbf{1}]$\alpha$& \textbf{1}(\textbf{1})[\textbf{2}]$\alpha$& $\alpha$& $\alpha$& $\cdots$& $\cdots$& $\cdots$& \ref{fig:DS39}\\
 44& 12236& 2014-12-12& 20:24& 241.0& 150$\times$100& N30& E71& W56&  120$^{+ 40}_{- 60}$&  2& \textbf{2}(\textbf{1})$\beta$& (\textbf{1})[\textbf{2}]$\beta$& $\beta$& $\beta$& $\beta$& $\beta$& $\beta$& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\cdots$& \ref{fig:DS40}\\
 45& 12230& 2014-12-11& 02:36& 178.8& 200$\times$145& S15& E40& W58&  150$^{+120}_{- 30}$&  1& $\beta$& $\beta$& $\beta\gamma$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\beta$& $\beta$& $\cdots$& $\cdots$& $\cdots$& \ref{fig:DS41}\\
 46& 12222& 2014-11-29& 06:36& 210.8& 320$\times$220& S20& E59& W55&  570$^{+450}_{-110}$& 11& $\alpha$& \textbf{1}$\beta\gamma$& \textbf{1}(\textbf{2})[\textbf{1}]$\beta\gamma$& \textbf{3}(\textbf{3})[\textbf{4}]$\beta\gamma$& $\beta\gamma$& $\beta\gamma$& \textbf{2}(\textbf{2})[\textbf{2}]$\beta\gamma$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta\gamma$& \textbf{2}(\textbf{1})$\beta\gamma$& \textbf{1}(\textbf{2})[\textbf{3}]$\beta\gamma$& $\cdots$& $\cdots$& \ref{fig:DS43}\\
 47& 12216& 2014-11-21& 20:24& 231.2& 240$\times$170& S13& E68& W59&  420$^{+220}_{-220}$&  8& \textbf{2}(\textbf{1})$\beta$& (\textbf{1})[\textbf{1}]$\beta\delta$& [\textbf{1}]$\beta\gamma$& $\beta\gamma\delta$& $\beta\gamma$& $\beta\gamma$& \textbf{4}(\textbf{3})[\textbf{3}]$\beta$& (\textbf{1})[\textbf{1}]$\beta$& \textbf{2}(\textbf{2})[\textbf{2}]$\beta$& $\beta$& $\cdots$& $\cdots$& \ref{fig:DS45}\\
 48& 12209& 2014-11-17& 02:48& 238.0& 320$\times$220& S15& E55& W75&  950$^{+150}_{- 50}$& 12& $\beta\gamma$& \textbf{1}$\beta\gamma\delta$& \textbf{2}(\textbf{3})[\textbf{1}]$\beta\gamma\delta$& \textbf{2}(\textbf{1})[\textbf{2}]$\beta\gamma\delta$& (\textbf{1})[\textbf{1}]$\beta\gamma\delta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta\gamma\delta$& \textbf{2}[\textbf{1}]$\beta\gamma\delta$& \textbf{2}(\textbf{3})[\textbf{2}]$\beta\gamma\delta$& \textbf{1}(\textbf{1})[\textbf{2}]$\beta\gamma\delta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta\gamma\delta$& (\textbf{1})[\textbf{1}]$\beta\gamma\delta$& $\cdots$& \ref{fig:DS46}\\
 49& 12187& 2014-10-20& 03:00& 244.4& 150$\times$150& S09& E67& W67&  190$^{+ 80}_{- 20}$&  1& $\alpha$& $\beta$& $\beta$& $\beta$& $\beta$& $\beta$& $\alpha$& $\beta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta$& $\alpha$& $\beta$& $\beta$& \ref{fig:DS48}\\
 50& 12178& 2014-09-30& 22:00& 248.6& 210$\times$140& S02& E70& W67&  120$^{+ 70}_{- 40}$&  4& $\alpha$& $\beta$& \textbf{1}(\textbf{1})$\beta$& [\textbf{1}]$\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\beta$& $\beta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta$& \textbf{2}(\textbf{2})[\textbf{2}]$\alpha$& $\alpha$& $\cdots$& \ref{fig:DS50}\\
 51& 12175& 2014-09-26& 23:12& 147.8& 270$\times$180& N16& E04& W77&  360$^{+220}_{- 90}$&  6& \textbf{1}(\textbf{1})$\beta\gamma$& \textbf{1}(\textbf{1})[\textbf{2}]$\beta\gamma\delta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta\gamma\delta$& \textbf{3}(\textbf{2})[\textbf{2}]$\beta\gamma\delta$& (\textbf{1})[\textbf{1}]$\beta\gamma\delta$& $\beta\gamma$& $\beta\gamma$& $\cdots$& $\cdots$& $\cdots$& $\cdots$& $\cdots$& \ref{fig:DS51}\\
 52& 12172& 2014-09-22& 17:00& 199.8& 340$\times$190& S11& E55& W54&  460$^{+ 30}_{- 50}$&  4& \textbf{1}(\textbf{1})[\textbf{1}]$\beta\delta$& $\beta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\beta\gamma$& \textbf{2}(\textbf{2})[\textbf{1}]$\beta\gamma$& [\textbf{1}]$\beta\gamma$& $\beta\gamma$& $\cdots$& $\cdots$& $\cdots$& \ref{fig:DS52}\\
 53& 12158& 2014-09-06& 01:24& 253.8& 220$\times$210& N16& E70& W69&  380$^{+210}_{- 40}$&  3& \textbf{2}$\alpha$& (\textbf{2})[\textbf{1}]$\beta$& \textbf{1}[\textbf{1}]$\beta\delta$& (\textbf{1})[\textbf{1}]$\beta\delta$& $\beta\gamma\delta$& $\beta\gamma\delta$& $\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\beta$& $\beta\gamma$& $\beta\gamma$& \ref{fig:DS53}\\
 54& 12149& 2014-08-31& 01:00& 251.2& 220$\times$150& N10& E69& W69&  190$^{+ 70}_{- 90}$&  1& $\beta$& $\beta\gamma$& $\beta\gamma$& $\beta\gamma\delta$& $\beta\gamma$& $\beta$& $\beta$& $\beta$& \textbf{1}$\beta$& (\textbf{1})[\textbf{1}]$\beta$& $\beta$& $\cdots$& \ref{fig:DS55}\\
 55& 12146& 2014-08-17& 20:12& 254.4& 130$\times$120& N09& E68& W72&  150$^{+ 70}_{-140}$&  4& \textbf{2}(\textbf{2})[\textbf{1}]$\alpha$& \textbf{1}(\textbf{1})[\textbf{2}]$\alpha$& $\alpha$& $\alpha$& $\beta$& $\beta$& $\beta$& $\beta$& $\beta$& \textbf{1}$\beta\delta$& (\textbf{1})[\textbf{1}]$\beta\delta$& $\beta\gamma\delta$& \ref{fig:DS56}\\
 56& 12135& 2014-08-08& 01:48& 249.8& 260$\times$170& N12& E69& W68&  170$^{+ 80}_{- 70}$&  2& \textbf{1}$\beta$& (\textbf{1})[\textbf{1}]$\beta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta\gamma$& $\beta\gamma$& $\beta$& $\beta$& $\beta$& $\beta$& $\beta$& $\beta$& $\cdots$& $\cdots$& \ref{fig:DS57}\\
 57& 12109& 2014-07-06& 03:00& 265.8& 250$\times$220& S08& E74& W73&  620$^{+310}_{-180}$&  5& $\alpha$& $\beta$& \textbf{1}$\beta\gamma$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta\gamma$& (\textbf{1})$\beta\gamma\delta$& [\textbf{1}]$\beta\gamma\delta$& $\beta\gamma\delta$& \textbf{3}(\textbf{3})[\textbf{2}]$\beta\delta$& [\textbf{1}]$\beta$& $\beta$& $\beta$& $\beta$& \ref{fig:DS58}\\
 58& 12108& 2014-07-05& 19:48& 238.8& 280$\times$185& S08& E65& W67&  560$^{+470}_{-270}$&  9& $\beta$& $\beta$& $\beta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta\gamma$& $\beta\gamma$& $\beta\gamma\delta$& \textbf{2}(\textbf{2})[\textbf{2}]$\beta\gamma\delta$& \textbf{2}(\textbf{2})[\textbf{2}]$\beta\gamma\delta$& \textbf{3}(\textbf{2})[\textbf{1}]$\beta\gamma\delta$& \textbf{1}(\textbf{2})[\textbf{3}]$\beta\gamma$& $\beta\gamma$& $\cdots$& \ref{fig:DS59}\\
 59& 12085& 2014-06-08& 02:36& 170.8& 300$\times$120& S20& E28& W64&  460$^{+280}_{- 30}$&  6& \textbf{1}$\beta\gamma$& (\textbf{1})[\textbf{1}]$\beta\gamma$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta\gamma$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta\gamma\delta$& $\beta\gamma$& \textbf{2}(\textbf{2})[\textbf{1}]$\beta\gamma$& \textbf{1}(\textbf{1})[\textbf{2}]$\beta\gamma\delta$& $\cdots$& $\cdots$& $\cdots$& $\cdots$& $\cdots$& \ref{fig:DS62}\\
 60& 12082& 2014-06-06& 10:48& 197.8& 315$\times$210& N16& E47& W60&  220$^{+ 50}_{- 60}$&  6& \textbf{3}(\textbf{3})[\textbf{2}]$\beta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta\gamma$& [\textbf{1}]$\beta\gamma$& $\beta$& $\beta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta$& $\beta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta$& $\cdots$& $\cdots$& $\cdots$& $\cdots$& \ref{fig:DS63}\\
 61& 12080& 2014-06-06& 03:24& 210.8& 300$\times$140& S12& E46& W69&  300$^{+270}_{- 40}$&  5& $\beta$& \textbf{2}$\beta$& (\textbf{2})[\textbf{2}]$\beta\gamma$& $\beta\gamma\delta$& $\beta\gamma\delta$& $\beta\gamma\delta$& \textbf{3}(\textbf{3})[\textbf{3}]$\beta\gamma\delta$& $\beta\gamma\delta$& $\beta\gamma\delta$& $\beta\gamma\delta$& $\cdots$& $\cdots$& \ref{fig:DS64}\\
 62& 12056& 2014-05-08& 02:24& 251.2& 300$\times$200& N05& E71& W67&  300$^{+110}_{- 50}$&  1& \textbf{1}$\beta$& (\textbf{1})$\beta\gamma$& [\textbf{1}]$\beta\gamma\delta$& $\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\beta$& $\beta$& $\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\cdots$& \ref{fig:DS65}\\
 63& 12055& 2014-05-08& 09:24& 244.8& 280$\times$140& N12& E69& W65&  330$^{+130}_{-120}$&  5& \textbf{1}$\beta$& $\beta$& \textbf{1}(\textbf{2})[\textbf{2}]$\beta$& \textbf{3}(\textbf{2})[\textbf{2}]$\beta$& (\textbf{1})[\textbf{1}]$\beta\gamma$& $\beta\gamma$& $\beta$& $\beta$& $\beta$& $\beta$& $\beta$& $\cdots$& \ref{fig:DS66}\\
 64& 12049& 2014-04-30& 13:24& 260.8& 270$\times$180& S07& E74& W69&  300$^{+120}_{-100}$&  2& $\beta$& $\beta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\beta$& $\beta\gamma$& $\beta\gamma$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta$& $\alpha$& $\cdots$& \ref{fig:DS67}\\
 65& 12034& 2014-04-11& 23:36& 230.8& 300$\times$145& N04& E63& W64&  250$^{+120}_{-150}$&  3& \textbf{1}(\textbf{1})$\beta$& [\textbf{1}]$\beta$& $\beta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta\gamma$& $\beta$& $\beta\gamma$& $\beta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta$& $\beta$& $\beta\gamma$& $\cdots$& $\cdots$& \ref{fig:DS68}\\
 66& 12005& 2014-03-16& 11:36& 251.8& 190$\times$160& N13& E71& W67&  220$^{+ 50}_{- 30}$&  1& $\alpha$& $\alpha$& $\alpha$& \textbf{1}(\textbf{1})[\textbf{1}]$\alpha$& $\beta$& $\beta$& $\beta$& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\cdots$& \ref{fig:DS70}\\
 67& 11976& 2014-02-10& 01:12& 273.8& 345$\times$150& S15& E78& W71&  240$^{+ 60}_{-130}$&  2& \textbf{1}$\beta$& \textbf{1}(\textbf{2})[\textbf{2}]$\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\beta$& $\beta$& $\beta$& $\alpha$& $\beta$& $\alpha$& \ref{fig:DS72}\\
 68& 11960& 2014-01-26& 13:00& 274.4& 185$\times$170& S15& E74& W75&  200$^{+110}_{- 60}$&  3& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\alpha$& $\beta$& \textbf{2}(\textbf{2})[\textbf{2}]$\beta$& $\beta$& \textbf{1}(\textbf{1})$\beta$& [\textbf{1}]$\beta$& $\alpha$& \ref{fig:DS74}\\
 69& 11944& 2014-01-04& 08:48& 199.6& 420$\times$280& S09& E53& W56& 1420$^{+140}_{-120}$& 12& $\beta\gamma$& \textbf{3}(\textbf{2})[\textbf{2}]$\beta\gamma$& \textbf{2}(\textbf{3})[\textbf{3}]$\beta\gamma\delta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta\gamma\delta$& \textbf{1}$\beta\gamma\delta$& \textbf{1}(\textbf{1})$\beta\gamma\delta$& \textbf{2}(\textbf{2})[\textbf{3}]$\beta\gamma\delta$& \textbf{2}(\textbf{3})[\textbf{3}]$\beta\gamma\delta$& $\beta\gamma\delta$& $\beta\gamma\delta$& $\cdots$& $\cdots$& \ref{fig:DS75}\\
 70& 11899& 2013-11-15& 04:12& 259.8& 260$\times$240& N06& E71& W72&  560$^{+200}_{- 50}$&  3& $\alpha$& \textbf{1}$\alpha$& (\textbf{1})[\textbf{1}]$\beta$& $\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\alpha$& $\beta$& $\beta$& \textbf{2}(\textbf{2})[\textbf{2}]$\beta$& $\beta$& $\alpha$& \ref{fig:DS78}\\
 71& 11893& 2013-11-10& 14:12& 251.8& 260$\times$150& S13& E71& W67&  240$^{+100}_{- 50}$&  3& $\alpha$& \textbf{1}(\textbf{1})$\alpha$& [\textbf{1}]$\beta$& $\beta$& $\beta$& $\beta$& $\beta$& $\beta\gamma$& \textbf{2}(\textbf{2})$\beta\gamma$& [\textbf{2}]$\beta\delta$& $\cdots$& $\cdots$& \ref{fig:DS79}\\
 72& 11890& 2013-11-05& 12:48& 155.8& 280$\times$240& S11& E57& W28&  910$^{+250}_{- 10}$&  5& $\beta\gamma$& \textbf{2}(\textbf{2})$\beta\gamma\delta$& \textbf{1}[\textbf{1}]$\beta\gamma\delta$& \textbf{1}(\textbf{2})[\textbf{2}]$\beta\gamma\delta$& [\textbf{1}]$\beta\gamma\delta$& $\beta\gamma\delta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta\gamma\delta$& $\beta\gamma\delta$& $\cdots$& $\cdots$& $\cdots$& $\cdots$& \ref{fig:DS80}\\
 73& 11877& 2013-10-19& 17:36& 252.8& 235$\times$190& S12& E69& W70&  330$^{+100}_{- 70}$&  5& \textbf{1}(\textbf{1})$\alpha$& \textbf{2}(\textbf{2})[\textbf{1}]$\beta$& [\textbf{2}]$\beta\gamma$& $\beta$& \textbf{1}(\textbf{1})$\beta$& \textbf{1}(\textbf{1})[\textbf{2}]$\beta\gamma\delta$& $\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\beta\gamma\delta$& $\beta\gamma$& $\beta\gamma$& \ref{fig:DS81}\\
 74& 11875& 2013-10-20& 18:48& 255.8& 375$\times$185& N07& E37& W70&  420$^{+270}_{-300}$&  4& $\beta$& $\beta\gamma$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta\gamma$& $\beta\gamma$& $\beta\gamma\delta$& $\beta\gamma\delta$& \textbf{3}(\textbf{3})[\textbf{2}]$\beta\gamma\delta$& [\textbf{1}]$\beta\gamma\delta$& $\beta\gamma\delta$& $\beta\gamma\delta$& $\beta\gamma\delta$& $\cdots$& \ref{fig:DS82}\\
 75& 11861& 2013-10-10& 20:12& 194.0& 310$\times$150& S10& E33& W74&  350$^{+290}_{- 50}$&  5& $\beta$& \textbf{1}(\textbf{1})$\beta$& \textbf{2}(\textbf{2})[\textbf{2}]$\beta$& [\textbf{1}]$\beta\gamma\delta$& \textbf{1}(\textbf{1})$\beta\gamma$& [\textbf{1}]$\beta\gamma$& $\beta\gamma$& \textbf{1}$\beta$& (\textbf{1})[\textbf{1}]$\beta\gamma$& $\cdots$& $\cdots$& $\cdots$& \ref{fig:DS83}\\
 76& 11818& 2013-08-12& 00:36& 219.8& 245$\times$160& S07& E00& W66&  270$^{+210}_{- 60}$&  3& \textbf{1}$\alpha$& (\textbf{1})[\textbf{1}]$\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\beta$& $\beta$& \textbf{1}(\textbf{1})$\beta\gamma\delta$& \textbf{1}(\textbf{1})[\textbf{2}]$\beta\gamma\delta$& $\beta\delta$& $\alpha$& $\cdots$& $\cdots$& \ref{fig:DS84}\\
 77& 11734& 2013-05-01& 02:36& 240.8& 300$\times$180& S18& E57& W73&  400$^{+ 50}_{-160}$&  6& \textbf{1}(\textbf{1})[\textbf{1}]$\beta$& \textbf{1}$\beta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta$& (\textbf{1})$\beta\gamma$& [\textbf{1}]$\beta\gamma$& $\beta\gamma$& $\beta$& \textbf{2}(\textbf{1})[\textbf{1}]$\beta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta$& (\textbf{1})$\alpha$& [\textbf{1}]$\alpha$& $\cdots$& \ref{fig:DS85}\\
 78& 11711& 2013-04-01& 22:24& 256.0& 200$\times$200& S17& E76& W63&  440$^{+ 90}_{-120}$&  3& $\beta$& \textbf{1}(\textbf{1})$\beta$& \textbf{2}(\textbf{1})[\textbf{1}]$\beta$& (\textbf{1})[\textbf{2}]$\beta$& $\beta$& $\beta$& $\beta$& $\beta$& $\beta$& $\beta$& $\alpha$& $\cdots$& \ref{fig:DS87}\\
 79& 11654& 2013-01-09& 21:48& 239.8& 450$\times$250& N08& E79& W53&  770$^{+510}_{-220}$&  7& \textbf{1}$\beta\gamma$& \textbf{1}(\textbf{2})$\beta\gamma$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta\gamma$& \textbf{3}(\textbf{2})[\textbf{2}]$\beta\gamma$& \textbf{1}(\textbf{2})[\textbf{3}]$\beta\gamma$& [\textbf{1}]$\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\beta\gamma\delta$& $\beta\gamma\delta$& $\beta\gamma$& $\cdots$& \ref{fig:DS90}\\
 80& 11640& 2013-01-01& 08:00& 184.2& 270$\times$175& N28& E30& W68&  220$^{+140}_{-100}$&  4& $\beta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta$& $\beta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta$& \textbf{2}(\textbf{2})[\textbf{2}]$\beta\gamma\delta$& $\beta\gamma\delta$& $\beta\gamma\delta$& $\cdots$& $\cdots$& $\cdots$& $\cdots$& $\cdots$& \ref{fig:DS91}\\
 81& 11623& 2012-12-01& 20:48& 265.8& 290$\times$120& N08& E74& W72&  150$^{+ 60}_{-200}$&  4& $\beta$& $\beta$& $\beta\gamma$& \textbf{1}(\textbf{1})$\beta\gamma$& \textbf{1}(\textbf{1})[\textbf{2}]$\beta\gamma$& $\beta$& \textbf{1}$\beta$& \textbf{1}(\textbf{2})[\textbf{2}]$\beta$& $\beta$& $\beta$& $\alpha$& $\alpha$& \ref{fig:DS92}\\
 82& 11598& 2012-10-22& 07:48& 265.8& 220$\times$170& S11& E71& W76&  330$^{+120}_{- 40}$&  3& \textbf{1}(\textbf{1})[\textbf{1}]$\beta$& $\beta$& $\beta\delta$& $\beta\delta$& $\beta\delta$& $\beta\delta$& \textbf{2}(\textbf{2})[\textbf{2}]$\beta\delta$& $\beta$& $\beta$& $\alpha$& $\alpha$& $\alpha$& \ref{fig:DS93}\\
 83& 11596& 2012-10-20& 16:12& 266.8& 310$\times$150& N07& E75& W72&  290$^{+120}_{- 40}$&  1& $\beta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\beta$& $\beta$& $\beta$& $\beta$& $\beta\gamma$& $\beta$& $\cdots$& \ref{fig:DS94}\\
 84& 11543& 2012-08-09& 21:48& 263.8& 230$\times$150& N21& E72& W71&  250$^{+ 20}_{- 70}$&  4& $\beta$& \textbf{1}(\textbf{1})$\beta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta\gamma$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta$& [\textbf{1}]$\beta$& $\beta\gamma$& $\beta\gamma$& $\beta\gamma$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta\gamma$& $\alpha$& $\beta$& $\cdots$& \ref{fig:DS96}\\
 85& 11520& 2012-07-08& 22:48& 191.6& 259$\times$181& S16& E50& W54& 1070$^{+150}_{-300}$& 15& \textbf{2}(\textbf{1})$\beta\gamma$& \textbf{1}(\textbf{2})[\textbf{3}]$\beta\gamma$& $\beta\gamma\delta$& \textbf{1}(\textbf{1})$\beta\gamma\delta$& \textbf{3}(\textbf{2})[\textbf{2}]$\beta\gamma\delta$& \textbf{2}(\textbf{3})[\textbf{2}]$\beta\gamma\delta$& \textbf{2}(\textbf{2})[\textbf{3}]$\beta\gamma\delta$& \textbf{4}(\textbf{4})[\textbf{5}]$\beta\gamma\delta$& $\beta\gamma\delta$& $\cdots$& $\cdots$& $\cdots$& \ref{fig:DS97}\\
 86& 11515& 2012-06-28& 08:48& 252.0& 390$\times$200& S17& E68& W69&  620$^{+420}_{-230}$&  3& \textbf{3}(\textbf{1})[\textbf{1}]$\beta$& (\textbf{2})[\textbf{2}]$\beta$& $\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\beta\gamma\delta$& $\beta\gamma\delta$& $\beta\gamma\delta$& $\beta\gamma\delta$& $\beta\gamma$& $\cdots$& \ref{fig:DS98}\\
 87& 11513& 2012-07-03& 08:48& 272.0& 190$\times$180& N16& E74& W74&  120$^{+ 40}_{-120}$&  1& $\alpha$& $\beta$& $\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\beta\gamma$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\beta$& $\alpha$& $\cdots$& \ref{fig:DS99}\\
 88& 11504& 2012-06-12& 08:00& 271.8& 300$\times$165& S17& E73& W75&  570$^{+510}_{-170}$&  7& $\beta$& $\beta$& \textbf{1}$\beta$& \textbf{1}(\textbf{2})[\textbf{2}]$\beta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta$& $\beta\gamma\delta$& $\beta\gamma\delta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta\gamma$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta\gamma$& \textbf{1}(\textbf{1})$\beta$& [\textbf{1}]$\beta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta$& \ref{fig:DS100}\\
 89& 11476& 2012-05-08& 10:48& 192.8& 365$\times$200& N10& E48& W57&  940$^{+340}_{-100}$&  7& \textbf{2}(\textbf{2})[\textbf{1}]$\beta\gamma$& \textbf{2}(\textbf{1})[\textbf{1}]$\beta\gamma\delta$& (\textbf{1})[\textbf{2}]$\beta\gamma\delta$& $\beta\gamma\delta$& $\beta\gamma\delta$& \textbf{2}(\textbf{1})[\textbf{1}]$\beta\gamma\delta$& \textbf{1}(\textbf{2})[\textbf{1}]$\beta\gamma\delta$& [\textbf{1}]$\beta\gamma$& $\beta$& $\cdots$& $\cdots$& $\cdots$& \ref{fig:DS101}\\
 90& 11460& 2012-04-21& 09:00& 203.8& 225$\times$130& N16& E42& W69&  300$^{+250}_{-150}$&  5& $\beta$& $\beta$& $\beta$& \textbf{1}$\beta$& \textbf{3}(\textbf{4})[\textbf{3}]$\beta$& [\textbf{1}]$\beta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta$& $\beta$& $\cdots$& $\cdots$& $\cdots$& $\cdots$& \ref{fig:DS103}\\
 91& 11384& 2011-12-22& 02:24& 273.8& 270$\times$185& N12& E76& W74&  330$^{+240}_{-150}$&  5& $\beta$& \textbf{1}$\beta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta$& (\textbf{1})[\textbf{1}]$\beta$& $\beta$& $\beta$& $\beta$& \textbf{2}(\textbf{1})[\textbf{1}]$\beta$& \textbf{1}(\textbf{2})[\textbf{2}]$\beta$& $\beta$& $\beta$& $\beta$& \ref{fig:DS105}\\
 92& 11339& 2011-11-03& 02:00& 277.8& 340$\times$220& N19& E79& W72& 1030$^{+440}_{-370}$&  5& (\textbf{1})[\textbf{1}]$\beta\gamma$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta\gamma\delta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta\gamma\delta$& $\beta\gamma\delta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta\gamma\delta$& \textbf{1}$\beta\gamma\delta$& (\textbf{1})[\textbf{1}]$\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\cdots$& \ref{fig:DS106}\\
 93& 11330& 2011-10-23& 23:48& 241.8& 360$\times$195& N08& E75& W58&  450$^{+240}_{- 50}$&  6& \textbf{2}(\textbf{1})$\beta$& \textbf{1}(\textbf{2})[\textbf{3}]$\beta$& \textbf{2}(\textbf{2})[\textbf{1}]$\beta\gamma$& \textbf{1}(\textbf{1})[\textbf{2}]$\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\beta\gamma$& $\cdots$& $\cdots$& \ref{fig:DS107}\\
 94& 11314& 2011-10-12& 06:48& 207.8& 190$\times$150& N27& E54& W56&  280$^{+ 50}_{- 50}$&  4& $\alpha$& \textbf{2}(\textbf{1})[\textbf{2}]$\beta$& (\textbf{1})$\beta$& $\beta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta$& \textbf{1}$\beta$& (\textbf{1})[\textbf{1}]$\beta$& $\beta$& $\beta$& $\cdots$& $\cdots$& $\cdots$& \ref{fig:DS108}\\
 95& 11302& 2011-09-23& 22:12& 267.2& 360$\times$225& N13& E73& W74&  840$^{+430}_{-230}$&  7& \textbf{2}(\textbf{1})$\beta\gamma$& \textbf{1}(\textbf{2})[\textbf{2}]$\beta\gamma$& \textbf{2}(\textbf{1})[\textbf{2}]$\beta\gamma\delta$& (\textbf{1})$\beta\gamma\delta$& \textbf{1}(\textbf{1})[\textbf{2}]$\beta\gamma$& $\beta\gamma\delta$& $\beta\gamma\delta$& \textbf{1}(\textbf{1})$\beta\gamma\delta$& [\textbf{1}]$\beta\gamma\delta$& $\beta\gamma\delta$& $\beta\gamma\delta$& $\beta$& \ref{fig:DS110}\\
 96& 11289& 2011-09-09& 18:36& 233.6& 190$\times$160& N22& E60& W65&  370$^{+ 70}_{- 60}$&  5& \textbf{1}$\beta$& (\textbf{1})$\beta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta$& \textbf{1}[\textbf{1}]$\beta$& (\textbf{1})[\textbf{1}]$\beta$& $\beta$& $\beta$& \textbf{1}$\beta$& (\textbf{1})[\textbf{1}]$\beta$& \textbf{1}(\textbf{1})[\textbf{1}]$\beta$& $\cdots$& $\cdots$& \ref{fig:DS111}\\
 97& 11263& 2011-07-30& 10:12& 228.8& 310$\times$155& N17& E63& W61&  510$^{+ 70}_{- 90}$&  4& \textbf{1}(\textbf{1})[\textbf{1}]$\beta$& \textbf{2}(\textbf{2})[\textbf{1}]$\beta$& \textbf{1}(\textbf{1})[\textbf{2}]$\beta$& $\beta\gamma\delta$& $\beta\gamma\delta$& $\beta\gamma\delta$& $\beta\gamma\delta$& $\beta\gamma\delta$& $\beta\gamma\delta$& $\beta\gamma\delta$& $\cdots$& $\cdots$& \ref{fig:DS112}\\
\end{longtable}
\end{landscape}
}}

